Theory of coupled ion-electron transfer kinetics

The microscopic theory of chemical reactions is based on transition state theory, where atoms or ions transfer classically over an energy barrier, as electrons maintain their ground state. Electron transfer is fundamentally different and occurs by tunneling in response to solvent fluctuations. Here, we develop the theory of coupled ion-electron transfer, in which ions and solvent molecules fluctuate cooperatively to facilitate electron transfer. We derive a general formula of the reaction rate that depends on the overpotential, solvent properties, the electronic structure of the electron donor/acceptor, and the excess chemical potential of ions in the transition state. For Faradaic reactions, the theory predicts curved Tafel plots with a concentration-dependent reaction-limited current. For moderate overpotentials, our formula reduces to the Butler-Volmer equation and explains its relevance, not only in the well-known limit of large electron-transfer (solvent reorganization) energy, but also in the opposite limit of large ion-transfer energy. The rate formula is applied to Li-ion batteries, where reduction of the electrode host material couples with ion insertion. In the case of lithium iron phosphate, the theory accurately predicts the concentration dependence of the exchange current measured by {\it in operando} X-Ray microscopy without any adjustable parameters. These results pave the way for interfacial engineering to enhance ion intercalation rates, not only for batteries, but also for ionic separations and neuromorphic computing.

==> misc.tex <==
\begin{itemize}
    \item {\color{blue} (DONE)} Say that ion and electron transfer are in several processes in nature and give examples. Finish with the methods used to describe them (BV-Marcus).
    \item {\color{blue} (DONE)} Start the description of ion transfer based on the BV and adsorption picture. Discuss Fig.1a and say the brief history on its development. Stress MZB on the development on consistent `non-eq' thermodynamics formulations.
    \item {\color{blue} (DONE)} Continue with the electron transfer picture and circulate the parts I have on the history on that.
    \item Motivate the importance of ion-electron reaction and discuss about important applications such as energy storage, biological and catalysis. Discuss a bit on the PCET and add the important references here - Koper, Sharron HS, Nocera etc. Conclude with the importance of having a framework for general ions and not only protons.
    \item Summarize with what we already show in this work.
\end{itemize}

A similar reaction mechanism to coupled ion-electron transfer is that of proton coupled electron transfer (PCET or CPET). As described in detail by Koper~\cite{Koper2013}, Saveant~\cite{Saveant2014}, Mayer~\cite{Mayer2004} and Hammes-Schiffer~\cite{Hammes-Schiffer2018}, there is a set of conditions where both the proton and the electron are transferred simultaneously. The main differences between our treatment for the concerted ion-electron transfer and PCET or other coupled ion-pairing electron transfer mechanisms~\cite{Saveant2008,Fukuzumi2012} are: i) herein, the ion motion is described classically, ii) the ionic coordinate we use is the actual physical distance between the reactant and the product states, while in other works it corresponds either to a solvent coordinate or to the bond length between the ion and its host molecule.

Moreover, our theory draws a connection between the charge transfer coefficient $\alpha$ with the electron-environment coupling. According to eq.~\ref{eq:CIET_linear_TST}, when the parabolas of the RedOx species are symmetric we find $\alpha=1/2$. In the case of asymmetric parabolas, $\alpha$ diverges from this value and can either be smaller or larger than $1/2$. More specifically, when electrons interact stronger with their environment at their oxidized compared to their reduced state $\kappa_O/\kappa_R>1$. Then, it is found that $\alpha>1/2$. In the opposite case, where the electrons are tightly bounded to their reduced state, our analysis concludes that $\alpha<1/2$.
